Leveraging SDN to Monitor Critical Infrastricture Networks in a Smarter Way

In critical infrastructures, communication networks are used to exchange vital data among elements of Industrial Control Systems (ICSes). Due to the criticality of such systems and the increase of the cybersecurity risks in these contexts, best practices recommend the adoption of Intrusion Detection Systems (IDSes) as monitoring facilities. The choice of the positions of IDSes is crucial to monitor as many streams of data traffic as possible. This is especially true for the traffic patterns of ICS networks, mostly confined in many subnetworks, which are geographically distributed and largely autonomous. We introduce a methodology and a software architecture that allow an ICS operator to use the spare bandwidth that might be available in over-provisioned networks to forward replicas of traffic streams towards a single IDS placed at an arbitrary location. We leverage certain characteristics of ICS networks, like stability of topology and bandwidth needs predictability, and make use of the Software-Defined Networking (SDN) paradigm. We fulfill strict requirements about packet loss, for both functional and security aspects. Finally, we evaluate our approach on network topologies derived from real networks.

==> 020-scenario.tex <==
\section{Reference Scenario}

In the context of an industry it is usually possible to distinguish two 
fundamental areas: a \emph{management component} and an \emph{industrial process 
component}. Although they are both fundamental for supporting the operation of a 
company, they are oriented at pursuing different sets of goals, listed in 
decreasing order of priority: for the 
management component it is important to ensure protection of information 
through encryption, to guarantee that no pieces of information are altered 
without the interested parties being able to detect it (integrity), and to 
support the continuous operation of a system even in the presence of faults 
(reliability).
Some of these goals also apply to the industrial process component, although 
with different priority: in this case it is very important to ensure 
uninterrupted operation of the supply chain (availability), while integrity and 
encryption are considered slightly less important.

While all the above mentioned goals are generally applicable to most elements 
of the industrial system (e.g., storage, control units), they are clearly more 
critical for the network infrastructure that supports it. In this paper we focus 
exactly on the network infrastructure, considering both the portion that 
pertains to the management component and the one that is related with the 
industrial process component, and assuming that all devices in 
the network are SDN-enabled.

There are several elements involved in the scenario outlined above. First of 
all, there are \emph{Programmable Logic Controllers} (PLCs), namely devices that 
read status information from sensors and are in charge to drive a set of 
actuators to perform a task for which they have been programmed in advance.
PLCs are connected to a \emph{Supervisory Control And Data Acquisition} (SCADA) 
system, from which they obtain instructions about how to set parameters or how 
to deal with ordinary or excepational operating conditions.
In our vision, the described elements are interconnected by a communication 
network consisting of SDN-enabled switches (\emph{datapaths}). In turn, all the 
datapaths are coordinated by a logical \emph{controller}, consisting of one or 
more pieces of software that realize different network functions. Finally, the 
network includes a \emph{detector}, namely a software that is able to inspect 
traffic and to perform the functions of an Intrusion Detection System (IDS).

Among the above mentioned components, we exploit SDN datapaths and the detector 
in order to pursue our main goal, which is to monitor the communication 
infrastructure used in the industrial system in order to enforce a dynamic 
protection of its operation even when large-scale architectures are involved.


General note: the most basic form of monitoring consists in counting packets 
(using, e.g., suitable flow entries). This is less effective in terms of anomaly 
detection but definitely more lightweight from the point of view of network load.


==> 060-DetAlgorithm.tex <==
\section{New Stream Treatment - DRAFT}



\subsection*{Backgroud}

We suppose to have a standard and critical streams. The critical ones are streams that we suppose to know in advance in according with the design of the critical infrastructure. Those streams are handle by the multi-commodity flow algorithm. Instead, the standard ones are unusual streams that we do not know in advanced and are potentially malicious so that they needed to be monitored.
The algorithm that we are going to propose aims to define how to treat the new not-critical stream in terms of the bandwidth to be allocated, the path of the standard and standard-monitored stream.
\todo[inline]{Check out if names of the streams that we've just been mentioned (critical, not-critical, mirrored) match with names used in the model section}



\subsection*{Problem Formulation.}

Define an algorithm that defines how the proposed detection system has to treat a not-critical new stream.
When a new stream occurs we carry out the following algorithm that has to define:
\begin{itemize}
\renewcommand{\labelitemi}{-}
\item Path of the standard stream.
\item Path of the standard-mirrored stream. 
\item The bandwidth assigned to the new standard and standard-monitored stream.
\item Observation point. The switch SDN-based where the standard-monitored traffic is generated. We suppose to be one.
\end{itemize}


\subsection*{Assumptions}


\begin{itemize}
\item We know the source $S$ and destination $D$ of the standard stream.
\item We know the topology of the network and the residual bandwidth of every link.
\item We have the detector $I$ that is in charge of inspecting packets.
\item We allocate the same bandwidth both for standard and for standard-monitored stream.
\end{itemize}



\subsection*{Idea - DRAFT}

For each switch of the topology $O$ we perform a Dijkstra's shortest path algorithm between:
\begin{enumerate}
\item $O-S$
\item $O-I$
\item $O-D$
\end{enumerate} 

Once that we have choose the 3-tuple $(O-S, O-I, O-D)$ we allocate bandwidth of the new standard and standard-monitored stream equal the half residual bandwidth of the link with the lowest value.

From the point of view of the security we prefer as a observation point the SDN-switch that is closest to the destination in order to better deal with MITM attack. In according to that we introduce a penalty to each switch that grows as much as the switch is more faraway from the destination.

We aim to provide an algorithm that balances security needs and shortest path in terms of hops number. Further, the algorithm aspires to avoid the complete saturation of links in order to increase the probability to be able to transfer traffic between every pair of node.



\subsection*{Input-Output}

\begin{itemize}
\item[] \textbf{Input.} \textit{Source $S$ and destination $D$ of the standard stream. Destination of the mirrored stream $I$ that we call Inspector. Topology of the network.}
\item[] \textbf{Output.} \textit{Path of the standard and standard-mirrored stream. Bandwidth of the new standard stream.}
\end{itemize}




\subsection*{Potential issues}

\begin{itemize}
\item[] Am I able to realize that a link is in common to all three paths?
\end{itemize}


